Scheduling Flows on a Switch to Optimize Response Times

We study the scheduling of flows on a switch with the goal of optimizing metrics related to the response time of the flows. The input to the problem is a sequence of flow requests on a switch, where the switch is represented by a bipartite graph with a capacity on each vertex (or port), and a flow request is an edge with associated demand. In each round, a subset of edges can be scheduled subject to the constraint that the total demand of the scheduled edges incident on any vertex is at most the capacity of the vertex. Previous work has essentially settled the complexity of metrics based on {\em completion time}. The objective of average or maximum {\em response time}, however, is much more challenging. We present approximation algorithms for flow scheduling over a switch to optimize response time based metrics. For the average response time metric, whose NP-hardness follows directly from past work, we present an offline $O(1 + O(\log(n))/c)$ approximation algorithm for unit flows, assuming that the port capacities of the switch can be increased by a factor of $1 + c$, for any given positive integer $c$. For the maximum response time metric, we first establish that it is NP-hard to achieve an approximation factor of better than 4/3 without augmenting capacity. We then present an offline algorithm that achieves {\em optimal maximum response time}, assuming the capacity of each port is increased by at most $2 d_{max} - 1$, where $d_{max}$ is the maximum demand of any flow. Both algorithms are based on linear programming relaxations. We also study the online version of flow scheduling using the lens of competitive analysis, and present preliminary results along with experiments that evaluate the performance of fast online heuristics.

==> AverageResponse/AvgPreliminaries.tex <==
We abstract the underlying network topology as an $m\times m$ non-blocking switch which we denote by $\mathbf{S}_m$. The switch has $m$ input ports, $m$ output ports and a link between each pair of input and output ports. Note that this switch is equivalent to a complete $m\times m$ bipartite graph. Furthermore, in this model, each vertex (port) $p$ has a capacity $c_p$. Edges, on the other hand, are assumed to have unlimited capacity.

Each flow $f$ is specified by a quadruple $(i_f,o_f,\sigma_f,r_f)$ consisting of an input port $i_f$, an output port $o_f$, a size $\sigma_f$, and a release time $r_f$. We denote the set of all flows by $F$. Given a valid schedule, let $c_f$ and $\rho_f$ denote the completion time and response time of flow $f$ respectively, where the response time, $\rho_f= c_f-r_f$, is the time the flow spends in the system. Moreover, for convenience, we define $\kappa_f$ to be the minimum capacity of the two ports used by $f$, and $F_p$ to be the set of all flows using port $p$.

In the discrete model, we will be working with weighted-matching schedules. That is, a schedule is a sequence of weighted matchings in the bipartite graph. The restriction is that, in each step, the number of flows incident to a port is at most the port's capacity. The completion time of a flow is the earliest point in time where it is delivered.

In the continuous model, we will be working with bandwidth functions. More precisely, a valid schedule provides a bandwidth function $b_{ft}: \mathbb{N}\rightarrow \mathbb{R}^{\geq 0}$ for each flow $f$ such that, at any point in time $t$, for any port $p$ the sum of bandwidths of flows that use $p$ is at most the port's capacity; i.e. $\sum_{f\in F_p} b_{ft} \leq c_p$. The completion time of a flow is, again, the earliest point in time where it is delivered.

In what follows, we will focus on the discrete model.

==> Rebuttal/reviews.tex <==
The SPAA 2020 rebuttal period is now open, and will extend until
23:59 AoE on Wednesday 15 April.

During this time, you will have access to the current state of
your reviews and have the opportunity to submit a response of
up to 1000 words.

* The response must focus on any factual errors in the reviews
and any questions posed by the reviewers. It must not provide
new research results or reformulate the presentation. Try to be
as concise and to the point as possible.

* The rebuttal period is an opportunity to react to the
reviews, but not a requirement to do so. Thus, if you feel the
reviews are accurate and the reviewers have not asked any
questions, then you do not have to respond.

* The reviews are as submitted by the PC members, without any
coordination between them. Thus, there may be inconsistencies.
Furthermore, these are not the final versions of the reviews.
The reviews will later be updated to take into account the
discussions at the program committee meeting, and we may find
it necessary to solicit other outside reviews after the
rebuttal period.

* The program committee will read your responses carefully and
take this information into account during the discussions. On
the other hand, the program committee will not directly respond
to your responses, either before the program committee meeting
or in the final versions of the reviews.

* Your response will be seen by all PC members who have access
to the discussion of your paper, so please try to be polite and
constructive.

The reviews on your paper are attached to this letter. To
submit your response you should log on the EasyChair Web page
for SPAA 2020 and select your submission on the menu.

Thank you again for submitting a paper to SPAA 2020,
- Mike Spear

----------------------- REVIEW 1 ---------------------
SUBMISSION: 147
TITLE: Scheduling Flows on a Switch to Optimize Response Times
AUTHORS: Hamidreza Jahanjou, Rajmohan Rajaraman and David Stalfa

----------- Overall evaluation -----------
This paper presents approximation algorithms for flow scheduling over a switch to minimize the average and the maximum response time (known as completion time in the non-theory literature). Both the results rely on resource augmentation to achieve some bounds in the offline case.

The paper is very well written and accessible to the practitioners of the area, even those who focus more on the applied side than theoretical aspects of the problem. I could follow most of the results and understand the high-level reasoning behind the choices.

Although great, as a more applied person who works in the area, I'd have preferred constant approximation factors because the total number of flows in a datacenter (n) can be quite large at any point in time. This makes the first results somewhat less impactful. Similarly, the second result essentially asks for doubling the capacity of each link to achieve optimal maximum response time; meaning, the network should run at 50% capacity. In practice, nowadays providers often want to run network at a higher utilization level. I found the 4/3 result as the most useful one because it gives practitioners a good target as to what to target for with their heuristics.

I thought that Section 5 could be improved significantly by considering more workloads, different load factors, etc. After the theoretical part of the paper, this section focusing on the online case comes across as half-hearted, because it is neither strong theoretically nor from a practical evaluation standpoint.


----------------------- REVIEW 2 ---------------------
SUBMISSION: 147
TITLE: Scheduling Flows on a Switch to Optimize Response Times
AUTHORS: Hamidreza Jahanjou, Rajmohan Rajaraman and David Stalfa

----------- Overall evaluation -----------
In this paper, the authors study the optimization of flow response times for a single switch. Flow response time is a central optimality criterion in practice, defined as the difference between the release and completion time of a flow, where the authors consider both average and maximum flow response time (response time is also known as sojourn or waiting time). The relevance of this paper goes beyond a single switch, as some popular data center architectures have full bisection bandwidth and hence fit the studied model.

The main result is a polynomial-time offline approximation algorithm, with a roughly logarithmic approximation ratio for the average response time, requiring capacity augmentation. Moreover, the authors also investigate maximum response time, showing it to be NP-hard to approximate without augmentation, and an optimal algorithm where the resource augmentation depends on the maximum flow demand. Both algorithms employ linear programming relaxations, and especially the first one seems interesting. As an addition, the authors also investigate the online version with some preliminary results, and simulate three online heuristics.

In total, the authors study an interesting and theoretically challenging problem, with practical applications and provide good non-trivial results, in a well-written paper. The main results stands out, but the other parts are nice and relevant additions.


Further comments:
- for future comparisons it would be nice to publicly release your simulator along with your algorithm implementations
- for your simulations, I think it could be nice to use a real data set as well. However, that might as well happen in e.g. a journal extension
- Lemma 5.2: here a reference to Section 5.E of [1] would be nice, as the idea is quite similar, even though the authors consider reconfigurable networks, but in the end, the setting applies here as well
- moreover, two recent papers that consider flow time in reconfigurable networks (again, similar setting, if reconfiguration time is ignored) will appear at INFOCOM 2020 [2], one about practical application of flow times in a multicast setting [3], and one about theoretical extensions of [1], in [4]. As the reconfigurable setting is conceptually similar to here, it could be nice to include [1,3,4] in the related work section.
- minor, but please make sure that single references etc. don't overflow and form the only content of a line, as in, e.g., page 2 ([8]) and 7 ((iv)).
- also minor, but please unify the reference styles, compare, e.g., [44] and [49]


[1] https://nam05.safelinks.protection.outlook.com/?url=https:%2F%2Fwww.cs.jhu.edu%2F~xinjin%2Ffiles%2FINFOCOM17_Owan.pdf&amp;data=02%7C01%7Cr.rajaraman%40northeastern.edu%7C806b3c14f3cb49ae8f0c08d7dfd00891%7Ca8eec281aaa34daeac9b9a398b9215e7%7C0%7C0%7C637223956920197058&amp;sdata=2GtRoppFbeDv64zVCU%2BaPUcQMY92u80txS1xVOq%2Fcv0%3D&amp;reserved=0
[2] https://nam05.safelinks.protection.outlook.com/?url=https%3A%2F%2Finfocom2020.ieee-infocom.org%2Faccepted-paper-list-main-conference&amp;data=02%7C01%7Cr.rajaraman%40northeastern.edu%7C806b3c14f3cb49ae8f0c08d7dfd00891%7Ca8eec281aaa34daeac9b9a398b9215e7%7C0%7C0%7C637223956920197058&amp;sdata=lX1Mna9ZWtKCCEfeahwenXElJPoWycLc%2B8JFPj9lXqI%3D&amp;reserved=0
[3] https://nam05.safelinks.protection.outlook.com/?url=https%3A%2F%2Feprints.cs.univie.ac.at%2F6257%2F11%2F2020-infocom.pdf&amp;data=02%7C01%7Cr.rajaraman%40northeastern.edu%7C806b3c14f3cb49ae8f0c08d7dfd00891%7Ca8eec281aaa34daeac9b9a398b9215e7%7C0%7C0%7C637223956920197058&amp;sdata=rm3acj%2BpNVblRDYBI23YXt%2F%2BhNsHR7Xi38Md56OD3Tc%3D&amp;reserved=0
[4] https://nam05.safelinks.protection.outlook.com/?url=https%3A%2F%2Farxiv.org%2Fabs%2F2001.07784&amp;data=02%7C01%7Cr.rajaraman%40northeastern.edu%7C806b3c14f3cb49ae8f0c08d7dfd00891%7Ca8eec281aaa34daeac9b9a398b9215e7%7C0%7C0%7C637223956920197058&amp;sdata=a6wNhHjyjbWiKkRO0TPUTkHKLm2gTT7fdD%2BsUm1y5BI%3D&amp;reserved=0


----------------------- REVIEW 3 ---------------------
SUBMISSION: 147
TITLE: Scheduling Flows on a Switch to Optimize Response Times
AUTHORS: Hamidreza Jahanjou, Rajmohan Rajaraman and David Stalfa

----------- Overall evaluation -----------
* Summary
This paper considers a flow scheduling problem on a switch, where each flow \(e\) corresponds to an input port \(p\), an output port \(q\), and a demand \(d_e\) for the amount of data that needs to transfer before we consider this flow to finish. Each port in the switch have a (possibly non-uniform) capacity. At each time slot, each flow can send more than one unit of data from input port \(p\) to output port \(q\), as long as the total data of flows incident on the same port does not exceed the capacity of this port. This paper focuses on flow time (a.k.a. response time), and considers two target function: average flow time and maximum flow time.

The authors provide an offline \(O(1 + O(\log (n))/c)\) approximation algorithm for unit flows, assuming an augmentation of \((1 + c)\) on port capacities. For maximum flow time, they prove it NP-hard to achieve 4/3 approximation without augmentation. An optimal offline algorithm is given assuming augmentation of \((2d_{\max} - 1\), where \(d_{\max}\) is the maximum demand of any flow. A preliminary study on the online version is also included, together with experimental evaluations.

* Merits

The overall approach is a time indexed LP similar to Garg and Kumar, but replacing the time indexed capacity constraint with a time interval capacity constraint for every interval in the form \((4(a-1), 4a]\). The main contribution in this paper is the repeated relaxation and reformation of the intervals in the iterated rounding. At first, the capacity constraint is on every consecutive 4 units of time. After some variables get integral value, they are ignored and a new set of longer intervals is calculated, and the capacity constraints are relaxed such that capacity constraint is only required for each interval as a whole. Such grouping is similar to recent breakthrough on single machine scheduling with release times, targeting weighted flow time. This method may be of independent interest for other problems targeting weighted flow time.

The maximum response time version takes advantage of an old result that for any LP where there is an absolute value upper bound on the sum of positive or negative entries on the same column, then we can compute a rounded solution that approximately satisfies the LP. The online version is more an attempt to attack online arrival, and plays as a connection to the experimental evaluation part. The evaluation part compared three heuristics: MaxCard, MinRTime, and MaxWeight. MaxCard gets a max cardinality matching each time, MinRTime gets a maximal weighted matching where the weight is the lateness so far for each edge. MaxWeight is also maximal weighted matching, this time the weight is the size of the queue on each port. Experiments show that MaxWeight performs the best overall. If the average number of incoming flows per port is greater than 1, then their differences are limited.

* Typos and minor fix
- On bottom right of page 2, related works, reference [16] is for general network topologies.
- Page 5, left column, first paragraph about iterative rounding: not clear what \(\{b^l_{et}\}_{e,t}\) means
- Page 5, left column, forth bullet, should be \(b^*_{et}\)
- Bullet 5, \(b_{et} \in I\) not defined.

==> TitlePage.tex <==
\begin{titlepage}
    \begin{center}
        \vspace*{1cm}
        
        % title
        {\Huge \textbf{Scheduling Flows on a Switch to Optimize Response Times}}
        
        \vspace{2cm}
        
        \textbf{Abstract}
        \vspace{.5cm}
        
        \setlength{\parskip}{.25cm}
        \setlength{\parindent}{0cm}
        
        \begin{adjustwidth}{2cm}{2cm}
            \input{Abstract}
        \end{adjustwidth}
        
        \vfill
    
    \end{center}
\end{titlepage}
